RX-ADS: Interpretable Anomaly Detection using Adversarial ML for Electric Vehicle CAN data

Recent year has brought considerable advancements in Electric Vehicles (EVs) and associated infrastructures/communications. Intrusion Detection Systems (IDS) are widely deployed for anomaly detection in such critical infrastructures. This paper presents an Interpretable Anomaly Detection System (RX-ADS) for intrusion detection in CAN protocol communication in EVs. Contributions include: 1) window based feature extraction method; 2) deep Autoencoder based anomaly detection method; and 3) adversarial machine learning based explanation generation methodology. The presented approach was tested on two benchmark CAN datasets: OTIDS and Car Hacking. The anomaly detection performance of RX-ADS was compared against the state-of-the-art approaches on these datasets: HIDS and GIDS. The RX-ADS approach presented performance comparable to the HIDS approach (OTIDS dataset) and has outperformed HIDS and GIDS approaches (Car Hacking dataset). Further, the proposed approach was able to generate explanations for detected abnormal behaviors arising from various intrusions. These explanations were later validated by information used by domain experts to detect anomalies. Other advantages of RX-ADS include: 1) the method can be trained on unlabeled data; 2) explanations help experts in understanding anomalies and root course analysis, and also help with AI model debugging and diagnostics, ultimately improving user trust in AI systems.

==> intro.tex <==
In this era of industrial big data, a massive amount of data is available to the public through various industries such as intelligent transportation \cite{8301555} \cite{doi:10.1137/1.9781611972740.23}, power grids \cite{8591773}, cloud computing \cite{7990488},  and finance \cite{lecun_deep_2015}. 
Knowledge extraction on these data is crucial for continuous improvements, process automation, and resilience improvements of these industrial systems \cite{8252775}. 
Even though the availability of data increases exponentially with time, this multi-variety data has many complexities such as incompleteness, high-dimensionality, noise, and they are rarely labeled \cite{7403935}.

To model these industrial systems reliably, it is necessary to capture only the relevant information from these high-dimensional feature spaces \cite{doi:10.1137/1.9781611972740.23} \cite{HINRICHS201925} \cite{REN2019121}.
Capturing relevant information are performed using various feature extraction and dimensionality reduction techniques. 
Extracting relevant features leads to high accuracy of models, together with reduction in number of features, results in improved overall efficiency of models \cite{ZABALZA20161}. 


%Further, the reliability of knowledge extraction methods generally deteriorates due to the curse of dimensionality \cite{REN2019121}.
%Therefore, to model these systems reliably, it is necessary to capture the relevant information from these high-dimensional feature spaces \cite{doi:10.1137/1.9781611972740.23} \cite{HINRICHS201925}.
%In the era of big data, it is necessary to understanding and modelling complex real world systems in diverse fields such as biomedical \cite{lecun_deep_2015}, astronomy \cite{doi:10.1137/1.9781611972740.23}, geography\cite{doi:10.1137/1.9781611972740.23}, smart grids \cite{8591773}, and natural language processing \cite{lecun_deep_2015}. 
%Modelling complex real world systems require capturing the relevant information from these high-dimensional data spaces \cite{doi:10.1137/1.9781611972740.23} \cite{HINRICHS201925}.

%Capturing relevant information are performed using various feature extraction and dimensionality reduction techniques. 

During last two to three decades, many dimensionality reduction and feature extraction methods have been proposed. Principal Component Analysis (PCA) is a widely used linear algorithm for dimensionality which preserves most of the variability of data in the subspace \cite{WANG2016232}. Linear Discriminant Analysis (LDA) is another popular supervised linear algorithm which maximize the class separation at subspace \cite{WANG2016232}.
However, linearity is a major disadvantage for both LDA and PCA.
Locally Linear Embedding (LLE) is another unsupervised dimentionality reduction technique which uses neighborhood preservation learning to generate subspace \cite{WANG2016232}. However, this method has high sensitivity for noise/outliars. 
Autoencoders (AEs) are another widely used as dimentionality reduction techniques, and proven to improve the robustness of feature learning \cite{SUN2016171} compared to other approaches.
Therefore, this paper mainly focuses on AEs.



% Less accurate in preserving global structure than ISOMAP ,Known to have difficulty on non-convex manifolds (not true of ISOMAP)

Deep Neural Networks (DNNs) were successfully used to convert these high-dimensional feature spaces into new embedded representations with relevant and robust features \cite{REN2019121}\cite{LANGKVIST201411}\cite{6279976}. 
Specially in real word settings, unlabelled data is abundant.
Further, labelling process is time-consuming, expensive, and requires the expertise of the data \cite{LANGKVIST201411}. 
Therefore, unsupervised deep learning algorithm based feature learning(feature extraction) has gained tremendous attention. 
The main idea of this process is to  capture  the  relevant information from noisy high-dimensional input data, by performing non-linear mapping to an embedded representation \cite{DBLP:journals/corr/abs-1712-07788} \cite{J3}  \cite{SUN2016171}.
Because the embedded representation only contains relevant information, we can potentially find a better separation between different data clusters. This effective transformation of the input data space to embedded space has been achieved through unsupervised deep learning methods such as deep autoencoders (AEs) \cite{DBLP:journals/corr/abs-1712-07788}. 

%Other advantages of AEs include replacing handcrafted feature learning \cite{LU2017377},  improve the robustness of feature learning \cite{SUN2016171}, and reduces the time and storage space through dimensionality reduction \cite{Hinton504}. Figure 1 shows the idea of unsupervised feature learning.

%Curse of dimensionality can be avoided by manually cleaning up these high dimensional data spaces \cite{REN2019121} \cite{LANGKVIST201411}.
%However, this process is time-consuming, expensive, and requires the expertise of the data \cite{LANGKVIST201411}. 
%Therefore, the alternative solution is to use unsupervised feature learning techniques to remove irrelevant information and to reveal hidden relationships that exist within data \cite{REN2019121,LANGKVIST201411,6279976}. 
%Recently, Deep Neural Networks (DNNs) were successfully used to convert these high-dimensional feature spaces into new embedded representations with relevant and robust features \cite{REN2019121}\cite{LANGKVIST201411}\cite{6279976}. 
%such as  deep  neural  networks (DNNs) to convert these high-dimensional feature spaces into a new embedded representations with relevant and robust features \cite{REN2019121}\cite{LANGKVIST201411}\cite{6279976}. 


% Add_later 
%Deep learning had become the primary techniques with the state-of-the-art performance in many areas including biomedical \cite{lecun_deep_2015,Litjens2016}, cyber-physical systems \cite{8591773}, natural language processing \cite{lecun_deep_2015}, space exploration \cite{lecun_deep_2015} and many more \cite{article1}, \cite{8669852}. 
%However, the success of deep learning has primarily concentrated on supervised learning where the training of the models is performed with a-priory knowledge about the data \cite{article1}, \cite{8669852}.
%%%The scarcity of labeled data in real word systems, has put more focus towards unsupervised deep learning algorithms \cite{DL2015}.
%Amount of labeled data available today is negligible compare to the availability and generation of unlabelled data. 
%Further, it has been found that the superior performance of supervised deep learning techniques has the limitation on depending on numerous labeled training data in order to achieve good generalization \cite{article1}. 
%This limitation has gained the focus towards unsupervised deep learning algorithms \cite{DL2015}.
%, where they can train with the abundance of real-world unlabeled data \cite{DL2015}. %Therefore, unsupervised learning predicted to be far more important in the long term \cite{DL2015}. 
%In unsupervised learning, the training of the models is performed without a-priori knowledge about the data, intending to extract meaningful information that exits within the data \cite{article1}.
%%%Traditionally, unsupervised learning was used for dimensionality reduction \cite{MOHAMED2019}, clustering \cite{JAIN2010651}, and association rules \cite{10.1007/978-3-319-91192-2_21}.
%Even though there is no clear categorization of unsupervised learning algorithms, most commonly they come under three categories: dimensionality reduction \cite{MOHAMED2019}, clustering \cite{JAIN2010651}, and association rules \cite{10.1007/978-3-319-91192-2_21}.
%Dimensionality reduction is the process of transforming high dimensional features into a new feature space, typically the dimension of the new feature space is significantly lower \cite{MOHAMED2019}. Clustering is the process of grouping data into meaningful topics \cite{MOHAMED2019}. 
%Further, dimensionality reduction is considered to be the very first step for clustering\cite{MOHAMED2019}. 
%Association rule mining is the process of discovering meaningful relationships among features of a dataset \cite{10.1007/978-3-319-91192-2_21}.   
%%%Recent advancement of unsupervised deep learning has gone far beyond these concepts.
%Recently, unsupervised deep learning algorithm based feature learning(feature extraction) has gained tremendous attention. 
%The main idea of this process is to  capture  the  relevant information from noisy high-dimensional input data, by performing non-linear mapping to an embedded representation \cite{DBLP:journals/corr/abs-1712-07788} \cite{J3}  \cite{SUN2016171}.
%Because the embedded representation only contains relevant information, we can potentially find a better separation between different data clusters. This effective transformation of the input data space to embedded space has been achieved through unsupervised deep learning methods such as deep autoencoders (AEs) \cite{DBLP:journals/corr/abs-1712-07788}. 
%Other advantages of AEs include replacing handcrafted feature learning \cite{LU2017377},  improve the robustness of feature learning \cite{SUN2016171}, and reduces the time and storage space through dimensionality reduction \cite{Hinton504}. Figure 1 shows the idea of unsupervised feature learning.


%the clustering and classification tasks perform better in embedded feature space than in input data space\cite{DBLP:journals/corr/abs-1712-07788}.   
%Recently, unsupervised deep learning algorithm  embedding the input data is projected into a latent space (unsupervised feature learning), results in better clustering/classification performance \cite{DBLP:journals/corr/abs-1712-07788}. 
%In this case, the quality of the classification process mainly depends on the quality of the embedded representation of input data, which allows better separation between different classes with high intro class similarity.
%This effective transformation of the input data space to embedded space has achieved through unsupervised deep learning methods such as autoencoders \cite{DBLP:journals/corr/abs-1712-07788}.
%These Deep Neural Networks (DNNs) consist of layers of stacked models which has the capability to do high-level feature abstraction compared to shallow neural network  \cite{8669852}, \cite{8591773}. 
%Other advantages of the deep neural network include the ability to deal with high-dimensional data, feature extraction by the model itself, and better generalization capability \cite{8591773}.

%Many recently proposed clustering/classification methods use latent representations which are generated through auto-encoders. 
%However, most of these methods use one single low-dimensional manifold to represent the input data space. 

Even though Deep learning had become the primary techniques with the state-of-the-art performance in many areas, they have the problem of vanishing gradient, i.e., when the network goes deeper, its performance gets saturated or even starts degrading rapidly. \cite{He_2016_CVPR}.
Because of this, the shallow counterparts can perform better than it is deep network \cite{He_2016_CVPR}. 
%Especially for unlabelled data, it is difficult to decide the optimal number of hidden layers in the DNN.
%In some cases, shallow counterparts can perform better than it is deep network dua to vanishing gradient \cite{He_2016_CVPR}. 
%As a result, when network goes deeper, its performance gets saturated or even starts degrading rapidly.
%Further, the use of one single low-dimensional manifold to represent data is one main weakness of the above-discussed methods because, for complex data, the embedded representations might lose the information through layers which are needed to separate all cluster types efficiently. 
A couple of years back, He et al. proposed residual blocks between layers to alleviate the problem of performance degradation \cite{He_2016_CVPR}.
%This is alleviated by introducing residual blocks where input is combined in the hidden layers \cite{He_2016_CVPR}. 
These networks are called as Resnets.


In this paper, we suggest using residual blocks in Autoencoder architectures (Resnet Autoencoders: RAE) for unsupervised deep feature extraction. 
Our hypothesis is that AEs with residual connections will improve feature extraction and dimensionality reduction capability of traditional stacked AEs. 
The paper has the following contributions:
\begin{itemize}
    \item Presents a deep neural network for unsupervised feature learning 
    \item Performance comparison between proposed architecture (RAE) and TAE based embedded representations, using different number of hidden layers on four different datasets. 
    \begin{itemize}
        \item Reconstruction errors were compared between AE and RAE.
        %\item K-Nearest neighbor (KNN) classification is performed using the embedded representations generated by pre-trained RAE and TAE.
        \item Time comparison was performed between : KNN classification on direct input, TAE based KNN classification, and RAE based KNN classification.
        \item Deep Embedded Clustering (DEC) was performed using trained RAE and TAE.
    \end{itemize}
   % \item Open challenges and future research directions.
    \item Performance comparison with other widely used dimensionality reduction methods
\end{itemize}

The rest of the paper is organized as follows: 
Section II presents the related work; Section III presents the RAE architecture; Section IV discusses the experiments and results, and finally, Section V presents the conclusions of the paper. 



==> relatedwork.tex <==
%The traditional concept of unsupervised learning was mainly limited to the idea of data clustering and association rule mining.
%The expansion of deep learning methods and data mining, combined with this era of big data has given a much broader perspective to traditional unsupervised learning.
%Therefore, unsupervised learning is used not only for clustering, but also for dimentionality reduction \cite{MOHAMED2019}, generative modelling \cite{NIPS2014_5423} \cite{DBLP:journals/corr/Goodfellow17}, auto-regressive modelling \cite{inproceedingsUL} \cite{CHEN201846} and unsupervised feature learning (deep embedded representation learning) \cite{2018arXiv180107648A}. 
%This section discuss on deep unsupervised feature learning which is the process of embedding the input space to an embedded space using deep neural networks.
%The main focus of this paper is concentrated on deep unsupervised feature learning which is the process of embedding the input space to an embedded space using deep neural networks.
%Many of  these  architectures perform AE based non-linear mapping of input data to a embedded space which is a higher level low-dimensional manifold.
%Therefore the rest of this section discusses the related works which uses AE based embedded representation learning. 

%https://dl.acm.org/citation.cfm?id=3306082
%https://arxiv.org/pdf/1606.05908.pdf
%https://arxiv.org/pdf/1606.05908.pdf

%With the arrival of the era of industrial big data, a massive amount of data is available from multiple and heterogeneous sources at a rapid rate \cite{7990488}.  
%Correspondingly, it is essential to develop algorithms that have the capability to extract valuable information from this massive datasets\cite{7990488}.
%However, these massive datasets can have redundant, irrelevant, and fault features \cite{7403935}.  
%Especially for clustering and classification tasks, the performance generally deteriorates due to the curse of dimensionality.
%%%The performance of clustering and classification tasks generally deteriorates due to the curse of dimensionality. 

%Rest of this section discusses recent advancements in AEs based unsupervised feature learning approaches. 

%%%Many of the recent classification tasks use different variants of AEs, to learn feature representation from high-dimensional input data, where the learned (extracted) features will provide good separability for classification tasks.
%%%In these cases, feature extraction will be performed in an unsupervised manner whereas classification will be performed on the extracted features, in a supervised manner.
%Feature extraction using variants of AEs has shown the following advantages: improve the robustness of feature learning \cite{SUN2016171}, non-linear feature extraction \cite{J3}, replacing handcrafted features with efficient algorithms for unsupervised feature learning \cite{LU2017377}, and reduces the time and storage space through dimensionality reduction \cite{Hinton504}.
%%%Compared to classification tasks, the AE based clustering approached has shown significant architectural advancements within the past decade. In the past, clustering and feature learning were performed sequentially \cite{2018arXiv180107648A} \cite{Ding:2004:KMC:1015330.1015408}. 
%where it embedded the input space to a latent space, and then perform clustering on the embedded space. 
%%%\cite{2018arXiv180107648A} \cite{Ding:2004:KMC:1015330.1015408}. 
%%%Recently, the idea of deep clustering was introduced where it performs join optimization of feature learning (dimensionality reduction) and clustering \cite{2018arXiv180107648A}.  


%(a).
%Guo at el. have pointed out that Xie at el.'s clustering loss may corrupt the embedded representation, resulting in meaningless features, harming the clustering performance \cite{Guo:2017:IDE:3172077.3172131}. 
%To address this issue, Guo at el.proposed Improved Deep Embedded clustering (IDEC) that focuses on preserving the local structure of the data. 
%The architecture of IDEC is presented in Figure \ref{DECnIDEC} (b).

\begin{figure}[]
  \centering
  \includegraphics[scale=0.385]{Figures/Serial_dec.pdf} %\\
 % \subfigure[]{\includegraphics[scale=0.5]{Figures/IDEC.pdf}}

  \caption{Deep Embedded clustering with autoencoders \label{DECnIDEC}}
\end{figure}

%In \cite{DBLP:journals/corr/YangFSH16}, Yang at el. proposed a very similar idea to IDEC which uses k-means cost in embedded space, as a prior to improve the embedded representation towards cluster friendly representation. Jiang at el. proposed Variational Deep Embedding (VaDE) which is a variational autoencoder based unsupervised generative clustering method \cite{DBLP:journals/corr/jiangZTTZ16}. 
%In \cite{DBLP:journals/corr/DizajiHH17}, Dizaji at el. has proposed Deep Embedded Regularized Clustering (DEPICT) which uses multi-layer convolutional autoencoders.  %Their approach also consists of joint optimization of clustering and reconstruction loss. 
%The clustering architecture proposed in \cite{6976982} is very similar to the idea presented in Figure \ref{DECnIDEC} (a). 
%They have imposed two constraints on embedded representation learning, namely locality-preserving and group sparsity constraints. 
%In \cite{LI2018161}, authors have presented a deep clustering approach using fully connected convolutional AEs. 
%They argue that the embedded representations extracted from an encoder, may not be discriminative enough for efficient clustering. 
%To overcome that, they have proposed a soft k -means model on top of the encoder to make a unified clustering model.
%In \cite{DBLP:journals/corr/abs-1712-07788}, authors have proposed a very interesting architecture where they have used a mixture of autoencoders, trained simultaneously via a composite objective function. 
%This jointly optimizes the reconstruction error and cluster identification error. Authors argue that this approach generates embedded representations that are more suitable for clustering.  

Given that deep models can learn better representations, the next  question was 
"Is learning better networks as easy as stacking more layers?". 
By answering this question, He at el. raised the awareness towards the problem of performance degradation \cite{DBLP:journals/corr/HeZRS15}. 
I.e., when the depth of the network increases, the performance of the network will start to saturate and eventually it can even deteriorates \cite{Zaeemzadeh2020NormPreservationWR}.
This is not caused due to over-fitting but vanishing gradient of deep neural networks \cite{Zaeemzadeh2020NormPreservationWR}.

This problem been addressed by various network designs networks such as ResNets \cite{DBLP:journals/corr/HeZRS15, DBLP:journals/corr/HeZR016}, Highway Networks \cite{10.5555/2969442.2969505}, and DenseNets \cite{8099726}. All these network uses the same design principle, i.e., skip connections or residual connections \cite{Zaeemzadeh2020NormPreservationWR}.
These networks with skip connections have consistently shown state-of-the-art performances in different neural network typologies \cite{DBLP:journals/corr/HeZRS15, 10.5555/2969442.2969505}.
Other advantages of skip connection includes better easier training \cite{Zaeemzadeh2020NormPreservationWR}, numerical stability and easier optimization \cite{article45} \cite{Zaeemzadeh2020NormPreservationWR}.
%skip connection enforces the norm-preservation during the training, leading to well-conditioning and easier training.
The ResNet architecture is presented in Figure \ref{fig:Resnet}.
Empirical evidence has shown  that these deep architectures with skip connections should not produce a large error than its shallow counterparts  \cite{DBLP:journals/corr/HeZRS15, DBLP:journals/corr/HeZR016}. 

As discussed in previous section, AEs are widely used dimentionality reduction techniques.
They have the capability to convert input data space into a cluster friendly feature space through non-linear transformations \cite{2018arXiv180107648A}. 
Recent approaches have shown that dimensionality reduction and representation learning techniques can be used to convert the input data space into a feature space where the clustering and classification tasks can be performed more efficiently compared to direct use of input data space \cite{2018arXiv180107648A}. This AE based deep embedded clustering approach was initially proposed by Song at el. in 2013 \cite{10.1007/978-3-642-41822-8_15}. 
They have proposed a new object function and embedded it in the autoencoder model.
This allows a joint optimization of the autoencoder's non-linear mapping (minimizing reconstruction error) and clustering (updating the cluster centers).  Xie at el. proposed Deep Embedded Clustering (DEC) method which simultaneously learns embedded representation and cluster assignments using deep neural networks \cite{DBLP:journals/corr/XieGF15}.
The idea of DEC is presented in Figure \ref{DECnIDEC}.

%As we discussed in the introduction, residual connections are introduced to TAE architecture.
%To alleviate this, we presents autoencoder architecture with identity shortcut connections for embedded representation learning.


In this paper, we hypothesis that performance degradation of deep neural networks affects the feature extraction and dimensional reduction capability of traditional stacked AEs.
Therefore, we present RAE architecture for deep embedded classification and clustering tasks, with the goal of improving feature extraction and dimensional reduction capability of traditional AEs.
We hypothesis that combining residual connections into stacked AE architecture will provide following complementary features:
\begin{itemize}
    \item Deep architecture will provide high level embedded representation learning capability 
    \item Residual connections will alleviate possible information loss when increasing the number of hidden layers. I.e., Improved resistance to performance degradation.
\end{itemize}


%This was answered in \cite{DBLP:journals/corr/HeZRS15} where they showed that, as the network goes deeper, its performance c starts degrading rapidly (the problem of vanishing/exploding gradients and performance degradation).
%They showed that this problem can be addressed by introducing "identity shortcut connections"or "residual connection" \cite{DBLP:journals/corr/HeZRS15}.
%one of the most successful ways of addressing this problem was by introducing "identity shortcut connections", proposed by He at el \cite{DBLP:journals/corr/HeZRS15}.



%Further in \cite{DBLP:journals/corr/HeZR016}, He at el has proposed refinement to the proposed architecture by introducing a pre-activation variant of residual blocks that allows gradients to flow through the shortcut connections. 
%This paper used these identity shortcut connection (residual connection) based autoencoders for unsupervised feature learning.

%https://link.springer.com/content/pdf/10.1007%2F978-3-642-41822-8_15.pdf



==> temp.tex <==
 unsupervised learning of phase transition from principal component analysis to variational auto encoders 
    About UL techs to learn features that descibe configurations of physical systems
    
    --Unsupervised deep embedding for cluster analysis--
    data-> lower D embedding then it ieteravively optimize the clustering objective
    cluster centers are learned in lower d space 
    SGD is performed wrt embedding of input data points and cluster centroids 
    
    --Deep clustering of Unsupervised Kearning of Visual Features--
    It train the convnet to predict pseudo lables(cluster centers), update the nestwork parameters by predicting pseudo labels. 
    
    -unsupervised Visual representation learning by context prediction--
    From large image, extract two ranodm patches and train CNN to predict the position of the second patch compare to the first patch. : model learn to recongize objects and their parts. 
    
    --context encoders: feature learning by in-painting--
    CNN trained to predict the context of an image region conditioned its surrounding.: CNN should understand the entire image context and hypothesis the missing region.Used reconstruction loss and adverserial loss.
    
    --Evolving Unsupervised Deep neural networks for leaning meaningful representations--
    DL performs good at learning meningful representations. However optimal architecture design and model parameter estimation is a problems. so evolutionay algos are preffered. Paper present a evolving Unsupervised DNN to learn meaningful representations efficienctl. it finds model architecture and parameter values by using gene coding approach. 
    
   --UNSUPERVISED REPRESENTATION LEARNING WITH DEEP CONVOLUTIONAL GENERATIVE ADVERSARIAL NETWORKS 2016--
   d deep convolutional generative adversarial networks (DCGANs), that have certain architectural constraints, and
demonstrate that they are a strong candidate for unsupervised learning.
    
    --Unsupervised Learning of Video Representations using LSTMs 2016--
    (LSTM) networks to learn representations of video sequences.
    
    --Early Visual Concept Learning with Unsupervised Deep Learning 2016--
    we propose an unsupervised approach for learning disentangled representations of the underlying factors of variation. : 1) we show the importance of
neuroscience inspired constraints (data continuity, redundancy reduction and statistical independence)
for learning disentangled representations of continuous visual generative factors; 2) we devise a
protocol to quantitatively compare the degree of disentanglement learnt by different models; and
3) we demonstrate how learning disentangled representations enables zero-shot inference and the
emergence of basic visual concepts, such as “objectness”.

    --Deep Predictive Coding Networks for Video Prediction and Unsupervised Learning 2016--
    we explore prediction of future frames in a video sequence as an unsupervised learning rule.
     a predictive neural network ("PredNet") architecture that is inspired by the concept of "predictive coding" from the neuroscience literature. These networks learn to predict future frames in a video sequence, with each layer in the network making local predictions and only forwarding deviations from those predictions to subsequent network layers. We show that these networks are able to robustly learn to predict the movement of synthetic (rendered) objects,
     

-Event-Based, Timescale Invariant Unsupervised Online Deep Learning With STDP 2018 -

In this work, we introduce a deep spiking convolutional neural network of integrate-and-fire (IF) neurons which performs unsupervised online deep learning with spike-timing dependent plasticity (STDP) from a stream of asynchronous and continuous event-based data.
In contrast to previous approaches to unsupervised deep learning with spikes, where layers were trained successively, we introduce a mechanism to train all layers of the network simultaneously.


-A deep learning framework for unsupervised affine and deformable image registration 2018 -
Unsupervised Deep Learning Image Registration (DLIR) ,
ConvNets are trained for image registration by exploiting image similarity analogous to conventional intensity-based image registration. After a ConvNet has been trained with the DLIR framework, it can be used to register pairs of unseen images in one shot.  

-Unsupervised Deep Representations for Learning Audience Facial Behaviors-2018 
 unsupervised learning approach for analyzing facial behavior based on a deep generative
model combined with a convolutional neural network
(CNN).We jointly train a variational auto-encoder
(VAE) and a generative adversarial network (GAN) to learn
a powerful latent representation from footage of audiences
viewing feature-length movies. We show that the learned
latent representation successfully encodes meaningful signatures
of behaviors related to audience engagement (smiling
and  laughing) and disengagement (yawning). 

--An Unsupervised Deep Learning Approach for Scenario Forecasts 2018-
a newly-developed unsupervised deep learning framework, the generative adversarial networks, to learn
the intrinsic patterns in historical renewable generation data.
Then by solving an optimization problem, we are able to quickly
generate large number of realistic future scenarios. 


-An Overview of Deep Learning Based Methods for Unsupervised and Semi-Supervised Anomaly Detection in Videos 2018-
. This article reviews the state-of-the-art deep learning based methods for video anomaly detection
and categorizes them based on the type of model and criteria of detection.
variational autoencoder (VAE) [1] , generative adversarial
networks (GANs) [2], Long Short Term memory networks (LSTMs) [3] , and others


-Clustering with Deep Learning: Taxonomy and New Methods 2018-  


\subsection{\textbf{Experiment 1: Classification }}
For this experiment, both TAE and RAE were trained using the hyper-parameters presented in Table \ref{HP_classifi}.
%The kernel sizes and optimizer details are attached in the appendix. 
The trained models were used to generate the encoded representation for the test datasets. 
These encoded representations were used for the classification using the K-Nearest Neighbor (KNN) algorithm.
I.e., after the encoder of each model together with KNN used as the classification network (TAE+KNN, RAE+KNN). 
Each experiment was repeated six times, and the average performances were recorded.

\subsubsection{\textbf{Hyper-parameters and architectural details}}
Hyper-parameters used for TAE+KNN and RAE+KNN are presented in Table \ref{HP_classifi}. 
%For this experiment, one residual connections from the input were added to the odd-numbered hidden layers.
Table \ref{HP_classifi}, column 2 represents the number of layers of each architecture together with number of neurons in each layer.
The number of hidden layers were increased from 1 to 12. 
For this experiment, one residual connection from the input were added to the hidden layer just before the last hidden layer.
Optimizer and K was selected through series of experimentation. The ones which gives the best accuracy is presented in the table.

%Input $x$ was converted to the same dimension as similar, given the hidden layer by adding a densely-connected neural network layer. 
%The Keras.layers.Add() function was used to add two layers and generated a single tensor, which will act as the input to the next hidden layer. 
%The number of epochs was kept at 50.


\subsubsection{\textbf{Classification Accuracy}}
Table \ref{ClaAcc} shows the classification accuracies obtained using the two models.
Single-layer models have only one hidden layer of neurons.
For all the datasets, the classification accuracy of at least one or more deep models (models with two or more layers) showed better accuracy compared to the single layers models.
Therefore, it can be inferred that deep models (models with two or more layers) have better performance compared to single-layer/shallow models. 
For all the datasets except for HAR, TAE+KNN/RAE+KNN based embedded representation classifications showed higher classification accuracy compared to KNN classification on direct input data.
This shows that TAE/RAE has the capability to convert input data to an embedded representation which is more suitable for the classification task. 
For HAR TAE/RAE embedded classification accuracy was 1.26\%, lower compared to the KNN classification on direct input data.
This might be able to alleviate by hyper-parameter tuning of RAE+KNN and TAE+KNN models.
Based on accuracies, experiments show that deep embedded representation based classification models have better or similar performance compared to direct input data classification on these four datasets. 

When increasing the number of hidden layers, the classification accuracy  increased at the beginning and then started to decrease gradually (Figure \ref{ClassAccuracyplots} and Table \ref{ClaAcc} ). 
For example, for the Reuters dataset, the classification accuracy of RAE+KNN was increasing until the fourth hidden layer and then decreased gradually. 
For all the tested models, when comparing the maximum accuracies of RAE+KNN and TAE+KNN, RAE+KNN showed almost similar or better performance for all datasets.

Figure \ref{fig:AccDis} shows the box plots for classification accuracy distribution for each dataset when increasing the number of layers. 
It shows that RAE+KNN has a low variance of accuracy as well as a higher mean accuracy value compared to the vanilla AE+KNN. 
Therefore, it can be inferred that RAE based embedded representations are less likely to under-perform when increasing the number of layers.
This observation supports our hypothesis. 




\begin{table}[t]
\centering
\caption{Time taken by different models for different datasets \label{Time}}
\begin{tabular}{l|l|l|l}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{l}{\textbf{Time (s)}} \\ \cline{2-4} 
                                  & KNN         & AE+knn     & RAE+knn     \\ \hline
\textit{\textbf{MNIST}}           & 6404.846    & 820.690    & 1212.981    \\ \hline
\textit{\textbf{Fasion\_MNIST}}   & 6435.077    & 491.194    & 634.604     \\ \hline
\textit{\textbf{Reuters}}         & 2120.964    & 229.043    & 372.162     \\ \hline
\textit{\textbf{HAR}}             & 89.997      & 28.774     & 35.573      \\ \hline
\end{tabular}
\end{table}


\begin{figure}[t]
  \centering
  \subfigure[]{\includegraphics[scale=0.28]{Figures/Loss20190921-192802_dataset_1_layers_4.pdf}}\quad
  \subfigure[]{\includegraphics[scale=0.28]{Figures/Loss20190921-201115_dataset_2_layers_4.pdf}} \\
  \subfigure[]{\includegraphics[scale=0.28]{Figures/Loss20190921-192517_dataset_4_layers_4.pdf}}
  \subfigure[]{\includegraphics[scale=0.28]{Figures/Loss20190921-194206_dataset_5_layers_4.pdf}}
  \caption{Change in reconstruction lost of the test data sets . (a) MNIST, (b) Reuters, (c) Fasion MNIST, and (d) HAR \label{ReconLoss}}
\end{figure}

\subsubsection{\textbf{Time comparison}}
Table \ref{Time} shows the computational time taken by embedded representation classification of TAE+KNN and RAE+KNN, and original input data classification using KNN algorithms.
Computation time was measured for training and testing on four different datasets. 
It can be seen that the KNN algorithm on original data took the highest time, whereas the TAE+KNN took the lowest time.
The KNN classification on original data takes the highest time due to the high-dimension of input data compared to the use of low dimensional embedded representations. 
RAE+KNN took a slightly higher computational time compared to TAE+KNN, which is expected due to extra computations of residual connection. 
However, these connections can be calculated in parallel.
RAE+KNN takes significantly lower time compared to KNN.
Therefore it can be inferred that RAE+KNN is efficient in terms of computational time and performance degradation compared to AE + KNN and KNN.
I.e., RAE+KNN gives a good trade-off between computational time and performance degradation. 


\begin{table*}[t]
\centering
\caption{Hyper-parameters of models \label{HP_clustering}}
\begin{tabular}{p{2cm}|p{10cm}|p{3cm}}
\hline
\textbf{Dataset}                        & \textbf{ Number of neurons in hidden layers}                                                                                                                                                                                                                                                                                          & \textbf{Number of Neurons in the last hidden layer} \\ \hline
\multirow{2}{*}{\textbf{MNIST}}         & \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}2 layers: 2000\\ 4 layers: 500, 500, 2000\\ 6 layers: 500, 500, 500, 500, 2000\\ 8 layers: 500, 500, 500, 500, 500, 500, 2000\\ 10 layers: 500, 500, 500, 500, 500, 500, 500, 500, 2000\\ 12 layers: 500, 500, 500, 500, 500, 500, 500, 500, 500, 500, 2000\end{tabular}} & 10                                                  \\ \cline{3-3} 
                                        &    &                                                     \\ \cline{1-1} \cline{3-3} 
\multirow{2}{*}{\textbf{Fashion MNIST}} &   & 10                                                  \\ \cline{3-3} 
                                        &   &                                                     \\ \cline{1-1} \cline{3-3} 
\multirow{2}{*}{\textbf{HAR}}           &   & 6                                                   \\ \cline{3-3} 
                                        &   &                                                     \\ \cline{1-1} \cline{3-3} 
\multirow{2}{*}{\textbf{Reuters}}       &   & 46                                                  \\ \cline{3-3} 
                                        &    &                                                     \\ \hline
\end{tabular}
\end{table*}



\subsubsection{\textbf{Reconstruction Loss comparison}}
Figure \ref{ReconLoss} shows the training reconstruction loss on the test data for both TAE and RAE against the number of epochs. 
For all datasets except for Reuters, RAE showed a lower reconstruction loss compared to TAE. The different behavior of Reuters can be due to the scarcity of the extracted features.  Therefore, it inferred that RAE has better capability to regenerate the input compared to TAE. 


\begin{table*}[t]
\centering
\caption{Hyper-parameters of models \label{HP_classifi}}
\begin{tabular}{p{2cm}|p{9cm}|p{1cm}|p{1cm}}

\hline
\multicolumn{1}{l|}{\textbf{Dataset}}              & \textbf{Hidden layers}  & \multicolumn{1}{l|}{\textbf{Optimizer}} & \multicolumn{1}{l}{\textbf{K parameter of KNN}} \\ \hline
\multicolumn{1}{l|}{\textbf{MNIST}}                & \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}1 layer: 64\\ 2 layers: 256, 64\\ 3 layers: 256, 128, 64\\ 4 layers: 256, 128, 128, 64\\ 6 layers: 256, 128, 128 ,128, 128, 64\\ \\ 8 layers: 256, 128, 128 ,128, 128, 128, 128, 64\\ \\ 10 layers: 256, 128, 128 ,128, 128, 128, 128, 128, 128, 64\\ \\ 12 layers: 256, 128, 128 ,128, 128, 128, 128, 128, 128, 128, 128, 64\end{tabular}} & \multicolumn{1}{l|}{adadelta}           & \multicolumn{1}{l}{5}                           \\ \cline{1-1} \cline{3-4} 
\multirow{2}{*}{}                                   &   &                                         &                                                  \\
                                                    &     &                                         &                                                  \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{\textbf{Fashion MNIST}}        &   & \multicolumn{1}{l|}{adadelta}           & \multicolumn{1}{l}{5}                           \\ \cline{1-1} \cline{3-4} 
\multirow{2}{*}{}                                   &   &                                         &                                                  \\
                                                    &  &                                         &                                                  \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{\textbf{Reuters}}              &  & \multicolumn{1}{l|}{adam}               & \multicolumn{1}{l}{10}                          \\ \cline{1-1} \cline{3-4} 
\multirow{2}{*}{}                                   &   &                                         &                                                  \\
                                                    &     &                                                  \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{HAR}}} & & \multicolumn{1}{l|}{adam}               & \multicolumn{1}{l}{5}                           \\ \cline{3-4} 
\multicolumn{1}{l|}{}                              &   &                                         &                                                  \\ \cline{1-2}\cline{3-4}
\end{tabular}
\end{table*}

@article{J3,
title = "Stacked Denoise Autoencoder Based Feature Extraction and Classification for Hyperspectral Images",
journal = "Journal of Sensors",
volume = "2016",
pages = "10",
year = "2016",
author = "Chen Xing, Li Ma, and Xiaoquan Yang"
}

